Revising Johnson's table for the 21st century

What does it mean today to study a problem from a computational point of view? We focus on parameterized complexity and on Column 16 "Graph Restrictions and Their Effect" of D. S. Johnson's Ongoing guide, where several puzzles were proposed in a summary table with 30 graph classes as rows and 11 problems as columns. Several of the 330 entries remain unclassified into Polynomial or NP-complete after 35 years. We provide a full dichotomy for the Steiner Tree column by proving that the problem is NP-complete when restricted to Undirected Path graphs. We revise Johnson's summary table according to the granularity provided by the parameterized complexity for NP-complete problems.

==> 06-FPT.tex <==
\section{FPT ideas}

We want to obtain an FPT algorithm for the dominating set problem restricted to undirected path graphs. Denote by $\DN(G)$ the domination number of $G$.

First, we present two propositions that help us reduce our graph. We say that $u$ and $v$ are \emph{twins} if $N[u] = N[v]$ (note that this implies that $uv\in E(G)$).

\begin{proposition}\label{prop:twin}
Let $G$ be a graph, and suppose that $u,v$ are twin vertices of $G$. Then:
\[\DN(G) = \DN(G-u).\]
\end{proposition}
\begin{proof}
First, let $S$ be a dominating set of $G-u$. Then either $v\in S$ or there exists $w\in S\cap N(v)$. In either case we get that $S$ is also a dominating set of $G$, i.e., $\DN(G)\le \DN(G-u)$. Now, let $S$ be a dominating set of $G$. Note that $|S\cap \{u,v\}|\le 1$; therefore we can suppose, without loss of generality, that $u\notin S$, in which case we trivially get that $S$ is also a dominating set of $G-u$. Hence $\DN(G-u)\le \DN(G)$.
\end{proof}

From now on we suppose that $G$ has no twin vertices. Observe that $u$ and $v$ are twin vertices if and only if $V(T_u) = V(T_v)$. Therefore, if $t = |V(T)|$, we get that $n = |V(G)| \le 2^t$. This means that if we can get an upper bound on $|V(T)|$ that depends only on $k$, say $|V(T)| = f(k)$, then we get a kernel of size $2^{f(k)}$. Also note that this kernel is also a kernel for connected dominating set.

The following proposition helps us on the task of bounding $t$.

\begin{proposition}
Let $G$ be an undirected path graph, and $(T,{T_u}_{u\in V(G)})$ be a minimal tree model for $G$. If $T$ has at least $2k+1$ leaves, then $\DN(G)>k$.
\end{proposition}
\begin{proof}
Let $\ell_1,\cdots,\ell_{2k+1}$ leaves of $T$, and let $v_1,\cdots,v_{2k+1}\in V(G)$ be such that $V(T_{v_i}) = \{\ell_i\}$ for each $i\in [2k+1]$. These vertices must exist because $T$ is a minimal tree model. Observe that for a vertex $u$ to dominate two distinct $v_i$ and $v_j$, we must have that $T_u$ is exactly equal to the path between $\ell_i$ and $\ell_j$ in $T$. Therefore, the best we can hope to dominate with $k$ vertices are $2k$ of the vertices in $\{v_1,\cdots, v_{2k+1}\}$.
\end{proof}

By the proposition above, we can suppose that $T$ has at most $k$ leaves \red{isso jah nao implica FPT pra Steiner Tree usando aquela ideia do Aleksander?}. It is known that the number of leaves on a tree equals 2 plus the number of vertices of degree bigger than~2. Therefore, if we denote by $t_{\ge 3},t_{2},t_1$ the number of vertices of degree at least~3, degree~2, and degree~1 in $T$, respectively, we get that $t_1 = t_{\ge 3}+2\le k$, which implies that $t \le t_2+ 2k-2$, i.e., it remains to bound the number of vertices of degree~2 in $T$.

Acho que limitar $t_2$ vai ser mais dificil, mas talvez ajude perceber que, se $P$ é um subcaminho de $T$ maximal tal que todo vertice interno tem grau~2, e $V_P = \{u\in V(G)\mid V(T_u)\cap V(P)\neq \emptyset\}$, entao $G[V_P]$ eh um grafo de intervalo e resolver dominating set em grafos de intervalo eh bem facil (olhar a referencia do Booth).
